Toward Fault-Tolerant Deadlock-Free Routing in HyperSurface-Embedded Controller Networks

HyperSurfaces (HSFs) consist of structurally reconfigurable metasurfaces whose electromagnetic properties can be changed via a software interface, using an embedded miniaturized network of controllers. With the HSF controllers, interconnected in an irregular, near-Manhattan geometry, we propose a robust, deterministic Fault-Tolerant (FT), deadlock- and livelock-free routing protocol where faults are contained in a set of disjointed rectangular regions called faulty blocks. The proposed FT protocol can support an unbounded number of faulty nodes as long as nodes outside the faulty blocks are connected. Simulation results show the efficacy of the proposed FT protocol under various faulty node distribution scenarios.

==> 3-topology.tex <==


As already outlined, the interconnect geometry design of choice for the HSF CN network is an irregular Manhattan-like topology~\cite{kouvaros2018formal} where the directionality of rows (and columns) alternates from one row (column) to the next, resembling a mesh topology where approximately half of its unidirectional links are missing. This network does not contain edge links that connect nodes found at the network periphery with their opposite-side topology nodes like in torus topologies termed ``end-to-end wraparound links'' (E2EWLs). This setup constrains hardware complexity, such as eliminating the introduction of two extra layers in order to accommodate such E2EWLs and transistors with higher signal drive to establish reliable data transmission. As a fair compromise, instead simple wraparound links called ``edge-wraparounds'' connect a pair of neighboring nodes residing on the same network peripheral column or row as shown in Fig.~\ref{fig:TopologyRouting} so as to improve routing adaptivity. Fig.~\ref{fig:TopologyRouting} shows such a $5 \times 5$ grid HSF topology, which forms a snippet of the $25 \times 25$ full-size HSF topology currently under development, as observed in our simulations of Section~\ref{sec:simulations}; said full-fledged topology is merely a recursion of the CN interconnect shown here.

%petrou2018asynchronous
Interconnectivity is critically affected by the clock-less/ asynchronously-operating circuits which have been opted to comprise the HSF CN architecture~\cite{nowick2015asynchronous}. This design choice is justified in \cite{petrou2018asynchronous} and concerns energy efficiency, cost and space savings, reduction in the implementation complexity associated with maintaining global clocks, and the interference induced by a clocked HSF EM layer. The technology used in the realization of the HSF limits the controller chip to 25 input/output signal pins as depicted in Fig.~\ref{fig:controller}. In order to carry out asynchronous communication among nodes, a four-way handshake protocol is utilized that requires three data pins to do so, where three pins are allocated for each input/output node channel. This restricts each node to two input and two output channels, as the rest of the controller pins are used for global signals, which gives rise to the Manhattan-like topology.   
\begin{figure}[t!]
	\centering
		\includegraphics[width= .4\columnwidth]{./figs/node.pdf}
		\vspace{-1mm}
	\caption{\small Pin allocation of the controller node and the layout of unidirectional input/output channels.}
	\label{fig:controller}
	\vspace{-5mm}
\end{figure}
%\input{figs/pin_allocation}

%Hence, nodes in the CN do not generate data packets but receive and forward them only.
Reconfiguration Directives (RDs) for each interconnected meta-atom are inserted via a \underline{G}ate\underline{W}ay (GW) connected to the lower left periphery of the network, while once a RD datum is received by a meta-atom, then its associated controller sends an \underline{ACK}nowledgement (ACK) message to the ACK GW connected at the topmost right corner of the CN. As such, each controller node, which comprises a single buffer to aid it convey RD along the network, either only consumes packetized RDs injected by the input GW and targeted toward it, or transfers them to the next node along a routing path, but never produces RD data, unlike in NoCs; however, as said, each node generates an ACK packet once a directive arrives, to be received by the ACK GW as RD receipt confirmation. 

%\magenta{We note, however, that in future implementations of the HyperSurface paradigm, controller nodes may also become message generators, e.g., in case the HSF is used for sensing purposes~\cite{liaskos2019absense}. Next, as current traffic patterns~\cite{saeed2019workload} indicate that faster metasurface responses may be required, the number of input gateways may also increase. These, may further strain the HSF CN in terms of traffic load, thus increasing the probability of contention, calling for architectural enhancements.}
%deadlocks.                 

The system-level resemblances between the HSF CN and typical 2-D NoC architectures suggest direct adoption of NoC methodologies to our controller network. While NoC routing scheme techniques can inspire equivalent methods for the HSF CN, the evident differences between the two systems necessitate a custom methodologies development for the HSF CN; crucially consider FT routing in fully-connected 2-D mesh-connected NoCs: as routing is \textbf{\textit{strongly coupled}} to said 2-D mesh topology on the basis of delivering packets to their destinations in a deadlock-/lievelock-free mode~\cite{DuatoBook,radetzki2013methods}, that is fundamentally different form the HSF CN Manhattan-like topology on account of connectivity and geometry, no FT routing for 2-D meshes can be adopted directly to our CN. Next, as neither virtual channels are used in the HSF controller nodes, most FT 2-D mesh routing protocols are rendered useless too~\cite{DuatoDeadFreeTheory}. Moreover, the HSF operates asynchronously whereas most NoCs are clocked, despite the presence of asynchronous-type signalling for flow control, such as using credits~\cite{DuatoBook}. Unlike in most wormhole-based NoCs, the HSF CN conveys complete packets that are not segmented into flits (i.e, flow-control units), the controllers are un-pipelined, and as said, where each contains just two input and two output ports with each comprising a single input buffer. 

% VS: moved from the intro to here, trimmed the intro
%At the system-level, there exists resemblance between Network-on-Chip-interconnected (NoC) multicore architectures and the HSF's CN geometry, in terms of miniaturization and overall layout.
%However, the adopted CN is marred by severe resource limitations, and as such exhibits a plethora of different operational characteristics vs. most conventional NoCs. First, the HSF CN operates clocklessly~\cite{petrou2018asynchronous}, as clocking introduces interference in the HSF's EM layer, where nodes locally exchange packets using localized asynchronous handshaking signals, without utilizing elaborate flow-control protocols such as wormhole credit-based flow-control~\cite{ duatoBook}; next, the single cycle (i.e., un-pipipelied) controllers (node equivalent in NoCs) each posses just two input and two output ports (i.e, channels/links) instead of four input and four output ports typical to 2-D mesh-connected NoCs, without the use of virtual channels~\cite{duatoBook}, and with just a single packet-sized buffer for each such input channel.

\begin{figure}[t!]
	\centering
		\includegraphics[width= .6\columnwidth]{./figs/topo2.pdf}
		\vspace{-1mm}
	\caption{\small A $5 \times 5$ HSF-embedded controller network topology with two packetized directives routing scenarios shown in solid blue and dotted orange links; the ACK path is shown in solid green.}
	\label{fig:TopologyRouting}
	\vspace{-5mm}
\end{figure}

%The two input and two output ports at each controller node lead to the alternating rows and columns directionality. At the network periphery, wraparound links are introduced to increase the level of adaptivity and robustness. However, inclusion of``traditional'' wraparound links that connect nodes found at the edges with their opposite topology nodes like in torus topologies, are avoided due to the additional hardware complexity that would be introduced. For example, two extra layers must be introduced to accommodate such wraparounds, as well as transistors with a higher signal drive that would establish the transmission over the distance of the wraparounds. Thus, in the considered topology edge-wraparounds connect edge nodes residing on the same column or row as shown in Fig. \ref{fig:TopologyRouting}

%The layout of the HSF controller network (HSF CN) comprise an irregular Manhattan like topology as shown in Fig. \ref{fig:TopologyRouting} where rows (and columns) represent unidirectional channels connected through edge-wraparound links. The direction of rows (columns) alternates between east and west (north and south) on every other row (column).  Below, we provide details and further exemplify the considerations which have led to this topology. 

%The current implementation technology node chosen for the controller chip has a limitation of 25 input/output signal pins as shown in Fig. \ref{controller} (a). The adoption of an asynchronous circuit leads to the implementation of a four-phase asynchronous handshake communication protocol between two controllers. The communication protocol requires three input/output pins per controller to transmit a single bit. In accommodating these restrictions, the design chosen provides two input channel endpoints and two output channel endpoints as shown in Fig \ref{fig:controller} (b). Such setup leads to the allocation of 12 pins for bit-by-bit communication (3 pins per channel endpoint) as shown in the Fig. \ref{controller} (c). The remaining 13 pins are used for configuring the meta-material and are allocated to global signals.

%this would require the construction of two more layers for wraparound circuits and, moreover, controllers at the edges would require transistors with a higher signal drive to achieve the transmission of a signal through such wraparound links. Instead, in the CN topology nodes that reside on the same edge row (column) are connected between them through \textit{edge wraparounds} as shown in Fig.\ref{fig:TopologyRouting}. 
%\hl{odd and even topologies} 

%The considered Manhattan-like topology can either have an even number of columns as shown in Fig. \ref{fig:TopologyRouting} (right) or an odd number of columns as shown in Fig. \ref{fig:TopologyRouting} (left). The two variations are referred to as even topology and odd topology, respectively. 

%The HSF can be composed of multiple metasurface tiles, the controller networks of which must be connected. Although the orientation of the CN does not affect the communication inside a single tile, it is important to pay attention to the CN orientation when tiling multiple surfaces. Surfaces with CNs of even topologies can simply be concatenated next to one another. However, a surface with network of an odd topology must be rotated by $90^\circ$ in order to be connected to another network (that is not rotated). Rotating every other network in a row of networks with odd topologies is necessary because of the unidirectional links of the network. In this paper we consider a network with an odd topology. However, the routing mechanism and the proofs presented are applicable for both network topologies.  

%The similarities between network on chip (NoC) systems and the HSF controller network suggest the adoption of NoC methodologies to our network. While NoCs routing techniques can inspire methodologies for the HSF CN, the significant differences between the two systems render existing NoC solutions inappropriate and necessitate new methodologies. The Manhattan like topology, as described above, is fundamentally different from the regular fully connected mesh topology characterizing most NoCs. In addition, the HSF CN is characterized by asynchronous operation, whereas most NoCs are clocked, despite the presence of asynchronous type signalling for flow control. Unlike NoCs, the HSF CN does not support virtual channels nor employ flow control units. 

%(\textcolor{blue}{Marios: What is left: literature review of NOCS routing related to our work.}

%These are Marios' suggestions, Thursday April 11, 2019 (via email):

%If possible can you please provide some guidelines as to the material that needs to be added to the current version of the paper so that we can work on it next week. I provide a possible breakdown below:

%\begin{itemize}
%\item A description about possible faults and their origin. We can use the following for guidelines (https://arxiv.org/pdf/1902.04509.pdf).
%\item Fault Tolerant Algorithm (the description that we have now to be completed by Taqua).
%\item Illuminating examples.
%\item Discussion on limitations with presentation of characteristic examples.
%\item Simulative Evaluation (As this might be the most time consuming part can you please provide guidelines and/or references on the simulation experiments to be conducted and on what simulator. Is Matlab ok or should we go for the custom built anylogic simulator?) 
%\end{itemize}


%As mentioned in the Introduction, the focus of this work is the development of a fault tolerant (FT) routing mechanism for the HSF CN. Authors in \cite{taghvaee2019fault} point out that the HSF system can be exposed to component failures throughout the manufacturing process or in the application environment. Individual random errors can be caused by fabrication mismatches which become mode likely to accrue in such miniature technologies. Spatially correlated fault on the other hand, can happen due to physical damages to the surface due to, for example, external attacks. The possibility of node or channel failures necessitate the development of a fault tolerant routing technique that suits the restrictions of the CN while efficiently delivers directives to healthy nodes in the network.  

%Many FT routing algorithms are build on the above principles to ensure seamless communication in NoCs, such as the FT scheme in \cite{vitkovskiy2013dynamic} which initiates a local detour every time a faulty node is encountered. As such, new path directives are added to the header which may create a large overhead. The method proposed in \cite{aisopos2011ariadne}, on the other hand, works proactively by disseminating routing data that is used to update routing tables right after a new fault is encountered, so as to bypass faulty links and routers. Another approach in \cite{wu2003fault} employs the notion of faulty blocks, where healthy links are victimized along with spatially close faulty links, to design a deterministic FT method where routed packets bypass such faulty blocks. Last, in an attempt to sustain good performance while avoiding deadlocks, several authors have utilized virtual channels \cite{radetzki2013methods}. This concept, however, is costly in terms of buffering, protocols, and control resources, which cannot be afforded in the HSF CN.



==> 5-southlast.tex <==

%\textcolor{red}{(VS: explain the rational for south-last routing: cause the entry gateway connected to the IoT device is in the right bottom corner (only source of data) and the recipient of ACKs GW is in the right top corner of the network, hence it make sense to route east then north, so south is the last resort in case we need to bypass a faulty block.)} \hl{Taqua: Done in section 4.1}

In this section we present the deadlock-free fault-tolerant routing mechanism which employs the turn prevention and faulty blocks concepts discussed in the previous section. This routing algorithm is based on a deadlock-free non-fault-tolerant version of the XY routing scheme proposed in \cite{saeed2018fault}. This version of the XY has been developed particularly for the topology under consideration, i.e. HSF CN. The considered XY version is referred to as XY-YX routing in this paper. 

XY-YX routing forwards a packet horizontally  then vertically then, if necessary, horizontally again. The method is aware of the unidirectionality of the rows and columns of the topology. Thus, when delivering a packet to a destination on an odd column, the packet is forwarded vertically through the column before the one on which the destination resides. Hence, the packets are never routed towards the west (i.e. one turn is never taken). For further details \cite{saeed2018fault}. This methods is deadlock free in a fault-free HSF CN topology. 

We employ turn prevention and FBs on top of the XY-YX routing in order to achieve deadlock freedom and fault tolerance. In a fault free environment packets follow XY-YX routing to reach their destinations. However, when faults are present and consequently FBs are formed packets are transmitted under a different routing mode around the fault block referred to as \textit{abnormal} routing. Abnormal routing decisions are mostly made at the boundary nodes of the FB. Packets are always routed clockwise around FBs such that all packets is only routed south when the destination is on the same column of the current column at a lower row. This way, no forbidden turns are taken throughout the routing process. It is important to mention here that $180$ degree turns at the edge wraparounds are blocked at all times. 

%------------------------------------------------------------------

\subsection{Routing of data packets}
As mentioned earlier in the paper, the input GW and the ACK GW are assumed to be connected to the bottom left corner and the top right corner of the network, respectively. Considering the location of the input GW and the assumption that there are no faults in the edges of the network, a data packet can only reach a faulty block from the southern boundary. In this case the destination must be north to the FB. In order to keep uniform rules for both data and ACK packets, the algorithm always routs around a FB in a clockwise direction. Thus, the packet must be routed west then north. Since the boundaries of FBs consist of two lines, the packet might reach an odd or an even column (i.e. the outer southern boundary line) based on the location of the fault. If the outer border is an odd row, the packet is routed west until the corner node of the FB is reached. However, if the outer border is an even row, thus directed towards the east, the packet is forwarded one hop towards the north to the inner border and then west towards the bottom left corner of the FB. A similar decision is made at the corner node, where the packet must reside on an even column to be routed north. If the inner west boundary is an odd column (i.e. directed towards the south), the packet is forwards one hop further to the west to the even column where it can be routed north until the top left corner of the FB. At the top left corner the packet simply follows XY-YX routing to reach its destination. Following this procedure, data packet do not take a forbidden turn at any point.  

%-------------------------------------------------------------------------------
\subsection{Acknowledgment Packets Routing}

Upon successful reception of a data packet, an ACK packet is generated and sent to the ACK GW connected to the top right corner of the network. In this work, we consider generating and sending the ACK packet from the node preceding the destination node in the packet path. This is to avoid the case of sending an ACK packet from a node of type 3 (a node residing on an odd row and an odd column) to the ACK GW, which requires taking the blocked turn SE.   

ACK packets are either routed east north, east or north depending on the location of the source of the ACK packet. As such, ACK packets reach FBs from the west boundary. To avoid taking forbidden turns the packet is routed clockwise around the block. Upon reaching the boundary line the algorithm locates the packet on the even column of the boundary such that it is routed to the north to the top left corner. Similar to the data packet, the ACK packet uses XY-YX from the top left corner to reach the ACK GW as shown in Fig. \ref{fig:rrouts}. 
%The procedure is summarized in Algorithm \ref{algo}.  


%begin{comment}
%\alglanguage{pseudocode}
%\begin{algorithm}[h]
%\small
%\caption{South-last routing}\label{algo}
%\begin{algorithmic}[1]
%\Procedure{$\mathbf{Routing \quad around \quad a\quad fault \quad block}$}{}
%\State The packet reaches a boundary node
%\State $x \gets \textit{current node column}$
%\State $y \gets \textit{current node row}$
%\State $x_d \gets \textit{destination node column}$
%\State $y_d \gets \textit{destination node row}$
%%\State $i \gets \textit{patlen}$
%%\BState \emph{top}:
%\If {$(x,y)$ is on the bottom left corner of FB}
%	\If{$y_d>y$} send up
%%	\Else \: follow XY
%	\EndIf	
%\ElsIf {$(x,y)$ is on a south boundary}
%		\If{$y_d>y$}
%			\If{$y$ is even} send up
%			\Else \: send left
%			\EndIf  
%		\Else \: follow XY
%		\EndIf 
%
%\ElsIf {$(x,y)$ is on a west boundary}
%		%\If{$y_d>y$}
%			\If{$x$ is even} send up
%			\Else \: send right
%			\EndIf  
%		%\EndIf
%\ElsIf{$(x,y)$ is on a north boundary} follow XY
%\Else \: follow XY
%\EndIf
%\State \textbf{Repeat}
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}
%\end{comment}


\begin{figure}[t]
	\centering
		\includegraphics[width=.40\textwidth]{./figs/FBrouts22.pdf}
		\vspace{-3mm}
	\caption{\small Routing around a faulty block: data packets in red and ACK packets in blue.}
	\vspace{-5mm}
	\label{fig:rrouts}
\end{figure}

\subsection{Deadlock and live-lock freedom of the south-last routing}

\begin{theorem}
South-last routing is deadlock free. 
\end{theorem}
\begin{proof}
A deadlock requires that four packets wait for each other in a cyclic path. Assume the packets $P_{i}$, where $i = 1,2,3$ and $4$, are in a deadlock. This requires one of the packets to be routed either SW or SE as shown in Fig. \ref{tturns}. The used turn model $Rule$ $1$ and $Rule$ $2$ prevent these two turns and 180 degree turns are blocked at edge wraparounds which rises a contradiction that proves the theorem.
\end{proof}

\red{VS: The entire next paragraph and proof are unnecessary.}
%\begin{theorem}
%South-last routing is livelock free.
%\end{theorem}
\begin{proof}
During normal mode, the offset in the x-dimension, $dx$, and the offset in the y-dimension, $dy$, are decreased by $1$ every time the packet takes a step in the respective direction. During abnormal routing, the packet can either reach the FB from the southern boundary in which case it is routed west, north then east or the packet can reach the FB from the western boundary. In the first case, $dx$ increases when the packet is routed west. However since the FB dimensions are finite this increase is temporary, and $dx$ is returned to $0$ when the packet is routed east at the end of the routing around the block. Moreover, $dy$ remains constant when the packet is routed west and east around the block and decreases when it is routed north. In the second case, the packet is routed north and then east. $dx$ remains constant when the packet is forwarded towards the north and decreases when the packet is routed east. $dy$ on the other hand decreases when the packet moves north and remains constant when the packet is routed east. Since the dimensions of all FBs are finite, presetting or increasing the value of any of the offsets is temporary and eventually $dx$ and $dy$ go to $0$ in a finite number of hops.   
\end{proof}


%------------------------------------------------------------------
\subsubsection{Faulty Blocks Overlapping}

In some cases, the overlap of faulty blocks can result in a deadlock or a live-lock. These cases involve one type of overlap, which is when the northern boundary of a FB is overlapping with the southern boundary of another FB. When these two boundaries overlap as depicted in the example of Fig. \ref{over1}, the south-last routing algorithm may force packets to break the turn model rules by taking a SE turn. In order to overcome this problem we eliminate the possibility of such an overlap by victimizing the overlapping boundary nodes and thus merging the overlapping FBs. This renders the combined FB a convex region (as shown in Fig. \ref{over2} right) that is easy to route around using the south-last routing mechanism.  

\begin{figure}[t!]
	\centering
		\includegraphics[width=.35\textwidth]{./figs/overlap1.pdf}
		\vspace{-2mm}
	\caption{\small Routing turns violation due to a problematic overlap of two faulty blocks.}
	\vspace{-3mm}
	\label{over1}
\end{figure}


 Note here that, any overlap between boarders other than northern with southern is not problematic. In addition, if the overlapping FBs have the same width and are exactly on top of each other, i.e. start on the same column and end on the same column as in Fig. \ref{over2}(left), their overlap is also not problematic. 
\begin{figure}[t!]
	\centering
		\includegraphics[width=.46\textwidth]{./figs/overlap2.pdf}
		\vspace{-2mm}
	\caption{\small Non-problematic overlap of two faulty block boundaries (Left), over-victimization to overcome problematic overlap (right). }
	\label{over2}
	\vspace{-3mm}
\end{figure}

==> figs/pin_allocation.tex <==
\begin{figure}
	\begin{center}
	\begin{tabular}{ccccc}
		\begin{tikzpicture}[scale=0.9]
			\draw		(0, 0) -- (0, 0);
			\draw[rounded corners]		(0.5, 0.5) rectangle (1.5, 1.5);
			\draw[fill]	(0.6, 0.6) circle (0.02);
			\draw[fill]	(0.8, 0.6) circle (0.02);
			\draw[fill]	(1, 0.6) circle (0.02);
			\draw[fill]	(1.2, 0.6) circle (0.02);
			\draw[fill]	(1.4, 0.6) circle (0.02);

			\draw[fill]	(0.6, 0.8) circle (0.02);
			\draw[fill]	(0.8, 0.8) circle (0.02);
			\draw[fill]	(1, 0.8) circle (0.02);
			\draw[fill]	(1.2, 0.8) circle (0.02);
			\draw[fill]	(1.4, 0.8) circle (0.02);

			\draw[fill]	(0.6, 1) circle (0.02);
			\draw[fill]	(0.8, 1) circle (0.02);
			\draw[fill]	(1, 1) circle (0.02);
			\draw[fill]	(1.2, 1) circle (0.02);
			\draw[fill]	(1.4, 1) circle (0.02);

			\draw[fill]	(0.6, 1.2) circle (0.02);
			\draw[fill]	(0.8, 1.2) circle (0.02);
			\draw[fill]	(1, 1.2) circle (0.02);
			\draw[fill]	(1.2, 1.2) circle (0.02);
			\draw[fill]	(1.4, 1.2) circle (0.02);

			\draw[fill]	(0.6, 1.4) circle (0.02);
			\draw[fill]	(0.8, 1.4) circle (0.02);
			\draw[fill]	(1, 1.4) circle (0.02);
			\draw[fill]	(1.2, 1.4) circle (0.02);
			\draw[fill]	(1.4, 1.4) circle (0.02);
		\end{tikzpicture}
		&
		\begin{tikzpicture}[scale=0.9]
			\draw[rounded corners]		(0.5, 0.5) rectangle (1.5, 1.5);
			\draw[->]	(0, 1) node[above] {\scriptsize input2} -- (0.5, 1);
			\draw[->]	(1.5, 1) -- (2, 1)  node[below] {\scriptsize output2} ;
			\draw[->]	(1, 0)  -- node[left] {\scriptsize input1} (1, 0.5);
			\draw[->]	(1, 1.5) -- node[right] {\scriptsize output1} (1, 2);
		\end{tikzpicture}
		&
		\begin{tikzpicture}[scale=0.9]
			\draw		(0, 0) -- (0, 0);
			\draw[rounded corners]		(0.5, 0.5) rectangle (1.5, 1.5);
			\draw[fill]	(0.6, 0.6) circle (0.02);
			\draw[fill]	(0.8, 0.6) circle (0.02);
			\draw[fill]	(1, 0.6) circle (0.02);
			\draw[fill]	(1.2, 0.6) circle (0.02);
			\draw[fill]	(1.4, 0.6) circle (0.02);

			\draw[fill]	(0.6, 0.8) circle (0.02);
			\draw[fill]	(0.8, 0.8) circle (0.02);
			\draw[fill]	(1, 0.8) circle (0.02);
			\draw[fill]	(1.2, 0.8) circle (0.02);
			\draw[fill]	(1.4, 0.8) circle (0.02);

			\draw[fill]	(0.6, 1) circle (0.02);
			\draw[fill]	(0.8, 1) circle (0.02);
			\draw[fill]	(1, 1) circle (0.02);
			\draw[fill]	(1.2, 1) circle (0.02);
			\draw[fill]	(1.4, 1) circle (0.02);

			\draw[fill]	(0.6, 1.2) circle (0.02);
			\draw[fill]	(0.8, 1.2) circle (0.02);
			\draw[fill]	(1, 1.2) circle (0.02);
			\draw[fill]	(1.2, 1.2) circle (0.02);
			\draw[fill]	(1.4, 1.2) circle (0.02);

			\draw[fill]	(0.6, 1.4) circle (0.02);
			\draw[fill]	(0.8, 1.4) circle (0.02);
			\draw[fill]	(1, 1.4) circle (0.02);
			\draw[fill]	(1.2, 1.4) circle (0.02);
			\draw[fill]	(1.4, 1.4) circle (0.02);


			\draw[->]	(0, 1.2) node[left] {\scriptsize data0} -- (0.6, 1.2);
			\draw[->]	(0, 1) node[left] {\scriptsize data1} -- (0.6, 1);
			\draw[<-]	(0, 0.8) node[left] {\scriptsize ack bit} -- (0.6, 0.8);


			\draw[->]	(1.4, 1.2) -- (2, 1.2) node[right] {\scriptsize data0} ;
			\draw[->]	(1.4, 1) -- (2, 1) node[right] {\scriptsize data1} ;
			\draw[<-]	(1.4, 0.8) -- (2, 0.8) node[right] {\scriptsize ack bit} ;

			\draw[->]	(0.8, 0) -- (0.8, 0.6);
			\draw[->]	(1, 0) -- (1, 0.6);
			\draw[<-]	(1.2, 0) -- (1.2, 0.6);

			\draw[->]	(0.8, 1.4) -- (0.8, 2);
			\draw[->]	(1, 1.4) -- (1, 2);
			\draw[<-]	(1.2, 1.4) -- (1.2, 2);

		\end{tikzpicture}

		\\
		{\scriptsize (a) Chip Pins}
		&
		{\scriptsize (b) Two inputs/outputs}
		&
		{\scriptsize (c) Communication: Pin allocation}
	\end{tabular}
	\end{center}
	\vspace{-2mm}
	\caption{\small (a) controller chip underside with pins placement, (b) single controller with its two unidirectional inputs and two output links, (c) CN chip pin allocation to facilitate external communication. \label{fig:controller}}
	\vspace{-5mm}
\end{figure}

